Learning the Number of Neurons in Deep Networks

Nowadays, the number of layers and of neurons in each layer of a deep network are typically set manually. While very deep and wide networks have proven effective in general, they come at a high memory and computation cost, thus making them impractical for constrained platforms. These networks, however, are known to have many redundant parameters, and could thus, in principle, be replaced by more compact architectures. In this paper, we introduce an approach to automatically determining the number of neurons in each layer of a deep network during learning. To this end, we propose to make use of structured sparsity during learning. More precisely, we use a group sparsity regularizer on the parameters of the network, where each group is defined to act on a single neuron. Starting from an overcomplete network, we show that our approach can reduce the number of parameters by up to 80\% while retaining or even improving the network accuracy.

==> ModelNet.tex <==
\section{Network Architectures}

\subsection{Representation Learning through Filter Compositions}
\label{sect:method}\vspace{-0.3cm}
\subsection{Decomposed Layers}
Our architecture builds upon the recent architecture proposed in~\citet{Alvarez:Arxiv2016}. The main property of that architecture consists of representing 2D kernels as compositions of consecutive 1D filters, see~\fig{fig:Diagram}. Instead of using a two steps training process where full kernels are learned and then approximated using low-rank filters, the architecture can be easily trained from scratch. As a result, decomposed networks are compact and require lower computational cost for training and testing while outperforming more complex networks.


In this paper, a convolutional layer refers to a 1D convolution while a decomposed layer as a layer consisting of two consecutive 1D convolutions with a non-linearity in-between.  'a layer' a set of two consecutive decomposed layers. Consider now a decomposed layer consisting of $C$ and $F$ input and output channels respectively. Let $\bar{v}$ and $(\bar{h})^T$ are vectors of length $d^v$ and $d^h$ respectively (representing the kernel size of each 1D feature map). We set in this paper $d^h=d^v\equiv d$, and $\varphi(\cdot)$ is a non-linearity set to rectified linear unit, ReLU~\cite{Krizhevsky_imagenetclassification}. Further, let us now denote $\mathbf{f}^i$ as the ith output kernel of the layer. Under this set up, $\mathbf{f}^i$  can be written as a linear combination of shared rectified filters,
\begin{equation}
\label{eq:dec}
a_i^1=\varphi(b_i^h + \sum_{l=1}^L{\bar{h}_{il}^T* [ \varphi( b_l^v + \sum_{c=1}^C{\bar{v}_{lc}*a_c^0})} ] )
\end{equation}
\noindent where $L$ represents the number of shared filters. According to~\citet{Alvarez:Arxiv2016}, $L$ must be large enough to provide sufficient diversity.


\subsection{Network Architecture}
Given the definition of a decomposed layer, our proposal concatenates eight of these layers as shown in~\fig{}, resulting in a total of 16 convolutional layers and 16 non-linearities. Our architecture follows conclusions in~\citet{Alvarez:Arxiv2016} and does not include fully connected layers except a linear classifier. We do not use pooling layers. Instead, and similarly to~\citet{ResNet2015} we use layers using a stride of $2$. As a consequence, the number of parameters in this basic model is approximately 12 million for Places2 (401 classes) and 13 million for ImageNet (1000 classes).







==> Results.tex <==
\section{Experiments on Bnet (VGG-B without Fully connected layer)}
\begin{itemize}
\item Influence of Batch size? Seems like large batch sizes makes a bit of a difference here. Importantly, removing the fully connected layer enables larger batch sizes.
\item Overall training is extremely slow ~ 5 days average on two titan-black with large batch size.
\item Can we show the benefits for learning with lower number of training data? (i.e., smaller batch sizes).
\end{itemize}

\begin{sidewaystable}[h]
%\begin{table}[h]
\scriptsize 
\centering
\caption{My caption}
\label{my-label}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{model} & \multicolumn{1}{c|}{Top-1} & \multicolumn{3}{c|}{C1} & \multicolumn{3}{c|}{C2} & \multicolumn{3}{c|}{C3} & \multicolumn{3}{c|}{C4} & \multicolumn{3}{c|}{C5} & \multicolumn{3}{c|}{C6} & \multicolumn{3}{c|}{C7} & \multicolumn{3}{c|}{C8} \\ \hline
myVD                        &                            & name  & $\tau$  & zeros & name  & $\tau$  & zeros & name  & $\tau$  & zeros & name  & $\tau$  & zeros & name  & $\tau$  & zeros & name  & $\tau$  & zeros & name  & $\tau$  & zeros & name  & $\tau$  & zeros \\ \hline
\end{tabular}
%\end{table}
\end{sidewaystable}




As expected, marginal accuracy improvements happen when using AlexNet and VGG in their original form. This is mainly due to the presence of the fully connected layer which constantly compensates for differences happening in previous layers. However, our proposal significantly reduces the amount of memory and parameters needed and consequently, speeds-up at test time.

Significant improvements are obtained when fully connected layers are completely removed.




\subsection{parameter sensitivity}
We focus now on the analysis of the sensitivity of the algorithm to the weights of the parameters. To this end, we represent in~\fig{} variations in performance and number of parameters (compared to a baseline) for different instances of our approach.

As shown, our algorithm systematically reduce the number of parameters while maintaining the performance. If additional savings are required, our approach significantly reduce the requirements while having minimal loss in performance (compared to optimal ones, that is, our best result).







==> oldExperiments.tex <==
\section{Experiments}

%\COMMENT{Talk about Speed, Memory savings (as parameters and channels), train-validation accuracy gap and performance}

%\COMMENT{A consideration to keep in mind is the fat that AlexNet and VGG architectures have been heavily tuned in the past and therefore marginal improvements  (although was shown that there is some redundancies in the parameters).}



\subsection{Architectures} 


\subsection{Datasets} 

We conduct experiments on three publicly available datasets. First, two large scale image classification datasets such as  ImageNet~\citep{DengDSLL009} and Places2~\citep{Places2} and then, we focus on character classification using ICDAR2003 dataset. ImageNet is a large-scale dataset with over $15$ million labelled images split into $22.000$ categories. We used the ILSVRC-2012~\citep{ImageNet} subset of images consisting of 1.2 million images for training and $50.000$ images for validation. Places2~\citep{Places2} is a large-scale dataset created specifically for training systems targeting high-level visual understanding~\citep{Places2} tasks, and consists of more than $10$ million images with $401$ unique scene categories. The database comprises between 5000 and 30000 training images per category which is consistent with real-world frequencies of occurrence. ICDAR dataset is dataset publicly available at~\citep{Jaderberg148} and consists of 185639 training and 5198 test samples. Training samples are character samples collected from a number of scene text and other synthesized datasets while the test set is from the ICDAR 2003 training set after removing all non-alphanumeric characters. Numbers correspond to the numbers in the dataset which are slightly different from the ones reported in the original paper (163222 training samples and 5379 test images).



\subsection{Experimental Setup} 

\textbf{ImageNet and Places2.} We consider three network structures: the AlexNetOWTBn in~\citet{Krizhevsky14} and the B-net in~\citet{Simonyan14c}(VGG-B) and the recently proposed Filter Decomposition~\citet{Alvarez16}. For AlexNetOWTBn (AlexNet from now on), we consider the one weird trick variation with batch normalization~\cite{IoffeS15}. B-net~\cite{Simonyan14c} is an instance of VGG structure consisting of $10$ convolutional layers with kernel sizes of $3\times 3$ and max-pooling every two of these convolutions. We use AlexNet$^C$ and BNet$^C$ to refer to variations of these architectures using only a fully-connected layer directly connected to the softmax layer. As filter compositions we consider Dec$_8$ consisting of $16$ convolutional layers of 1D kernels. For fair comparison, all models including baselines are trained from scratch on the same computer using the same seed and the same framework. More specifically, we use the torch-7 multi-gpu framework~\cite{Collobert_NIPSWORKSHOP_2011} on a Dual Xeon 8-core E5-2650 with 128GB of RAM using three Kepler Tesla K20 GPUs in parallel. All models are trained for a total of $55$ epochs with $12000$ batches per epoch and a batch size of $96$, $48$ and $180$ for AlexNetOWTBn, B-net and Dec$_8$ respectively. These variations in the batch size are mainly due to memory and training time limitations in the first two models. Data augmentation is done through random crops where necessary and random horizontal flips with probability $0.5$. Please note that other training approaches may use different data augmentation techniques such as color augmentation~\cite{Krizhevsky_imagenetclassification}. 




\textbf{ICDAR2003 Character Recognition.} For this dataset we consider a similar architecture as in~\cite{Jaderberg14b} consisting of three convolutional layers and a fully connected layer directly connected to the softmax output. We use max-pooling between layers instead of the maxout layer used in~\cite{Jaderberg14b}. In addition, instead of 2D kernels we consider decompose layers using 1D kernels (that is, we replace kernel of size $9\times 9$ by two consecutive convolutional layers of size $9\times 1$ and $1\times 9$. We train each network on a single Tesla K20m GPU for a total 45 epochs with a batch size of 256 and 1000 iterations per epoch. The learning rate is set to an initial value of 0.1 and multiplied by 0.1 in the second, seventh and fifteenth epochs and we use a momentum of 0.9. As previously, all models are trained from scratch. 

\textbf{Evaluation} We measure classification performance as the top-1 accuracy using the center crop, named \textbf{Top-1}. We also provide training-validation accuracy gap plots, named \textbf{Train-val gap}. This plot demonstrates the evolution of the difference between train and validation accuracy as the training proceeds~\cite{Batra:ICLR2016}. The expected behavior of this plot is a slight positive slope as training proceeds. A network with only a moderate amount of overfitting would produce a gentle slope while a significantly overfitting process would exhibit a steeper slope, that is, a larger gap between train and validation accuracy.

We provide results as follows: We consider as baselines the structures publicly available. Then, we include experimental results in pairs: first those obtained for variations of the model without without regularization terms and second, results our model selection proposal is taken into account.

\NEW{In our results, we use \textbf{neuron} to refer to the percentage of neurons set to zero, that is, neurons whose parameters are all set to zero. We use \textbf{group-wise sparsity} to refer to the percentage of parameters included in the neurons set to zero. We use \textbf{within-group sparsity} to refer to the percentage of parameters set to zero as a direct consequence of sparse penalties. That is, parameters in neurons set to zero plus additional parameters set to zero in neurons with at least one non-zero parameter. An equal percentage for within-group and group-wise means the only parameters having a zero value are those in neurons whose parameters are all zero. Finally, we use \textbf{total-induced} to refer to the total number of parameters being set to zero, including those in the last fully connected layer induced by the zeros in the last convolutional layer.}



\subsection{Results}
% \begin{figure}
%   \begin{minipage}[b]{0.40\linewidth}
%     \centering
% \includegraphics[width=\textwidth]{./figs/Bnet.png}
%     \par\vspace{0pt}
%   \end{minipage}%
% \hspace{-0.75cm}  \begin{minipage}[b]{0.40\linewidth}
%     \centering%
%     \begin{tabular}{ |l|c| }%
%       \hline%
%       \multicolumn{2}{|c|}{Saving Percentages} \\%
%       \hline \hline
%     neuron& 12.70\%\\
%     group-wise& 13.59\%\\
%     within-group& 13.59\%\\
%     total-induced & 25.58\%\\
%     \hline
%     \end{tabular}%
%     \par\vspace{0pt}
%   \end{minipage}
% \caption{Example results on ImageNet using BNet.}
% \label{fig:BNet} 
% \end{figure}


\begin{figure}
\begin{center}
\begin{minipage}[t]{.35\linewidth}
\vspace{0pt}
\centering
%\includegraphics[width=\textwidth]{./figs/Bnet.png}
\end{minipage}%
\begin{minipage}[t]{.25\linewidth}
\vspace{0pt}
\centering
\begin{tabular}{ |l|c| }%
      \multicolumn{2}{c}{}\\
      \hline%
      \multicolumn{2}{|c|}{AlexNet on ImageNet} \\%
      \hline \hline 
     &\multicolumn{1}{c|}{AlexNet512}\\%
     \hline
    neuron& 19.48\%\\
    group-wise& 22.52\%\\
    within-group& 22.52\%\\
    total-induced& 21.97\%\\
    \hline
    relative acc. & 0.2\%\\
    \hline      
    \end{tabular}%
\end{minipage}
\end{center}
\caption{Experimental results for AlexNet on ImageNet. This particular instance maintains the double fully connected layer as originally suggested in~\citep{Krizhevsky14}. Interestingly, when training without constraining the network, this architecture quickly overfits and the validation accuracy drops after thirty five epochs. Contrary, as a result of our algorithm, our proposal not only reduces significantly the number of parameters but also avoids overfitting.}
\label{fig:AlexNetConImageNet} 
\end{figure}


\begin{figure}
\begin{center}
\begin{minipage}[t]{.4\linewidth}
\vspace{0pt}
\centering
\hspace{-0.05cm}\includegraphics[width=\textwidth]{./figs/Dec8-768.png}
\end{minipage}%
\begin{minipage}[t]{.6\linewidth}
\vspace{0pt}
\centering
\hspace{-0.250cm}\begin{tabular}{ |l|c|c|c|c| }%
      \multicolumn{5}{c}{}\\
      \hline%
      \multicolumn{5}{|c|}{DecomposeMe on ImageNet (in \%)} \\%
      \hline \hline 
      &\multicolumn{1}{c|}{Dec$_8$}&\multicolumn{2}{c|}{Dec$_8$-$640$}&\multicolumn{1}{c|}{Dec$_8$-$768$} \\%
      \cline{2-5}
     &\multicolumn{1}{c|}{GS}&\multicolumn{1}{c|}{S-GS}&\multicolumn{1}{c|}{GS}&\multicolumn{1}{c|}{GS} \\%
     \hline
    neuron& 3.39& 12.42 & 4.02&26.83\\
    group-wise& 2.46& 13.69 & 4.22&31.53\\
    within-group& 2.46&22.72 & 4.22&31.63\\
    total-induced& 2.82&23.33& 10.83&32.26\\
    \hline
    relative acc. &0.01 & 0.94 &2.45 &-0.02\\
    \hline      
    \end{tabular}%
\end{minipage}
\end{center}
\caption{Experimental results for Dec$_8$-$640$ on ImageNet (640 neurons per layer instead of 512).\TODO{ADD Test Speed / Memory numbers}}
\label{fig:Dec640OnImageNet} 
\end{figure}
%9.89% 4.50% 4.63% 4.63%
%2.82% 3.39% 2.46% 2.46% -> no improvement
%    neuron& 3.39\%& 12.42\% & 6.32\%&26.83\%\\
%    group-wise& 2.46\%& 13.69\% & 7.24\%&31.53\%\\
%    within-group& 2.46\%&22.72\% & 10.44\%&31.63\%\\
%    total-induced& 2.82\%&23.33\%& 11.95\%&32.26\%\\

We notice a significant difference in the training validation accuracy gap when applying our regularization technique. For instance, for DecomposeMe$_8$-$768$ which reduce up to 32.2\% the number of parameters, the training-val. gap experiments a relative reduction of 28.5\% (from 14\% to 10\%) which suggests networks trained using our approach have better generalization abilities even using fewer parameters. 


 \begin{table}[!t]
 \caption{Top-1 accuracy results for our method and several state-of-the art architectures on ImageNet.}\label{tab:ImageNet}
 \centering
 \begin{minipage}[t]{.5\linewidth}
\begin{tabular}{ |l|c| }%
  \hline%
      \multicolumn{2}{|c|}{Top-1 acc (\%) on ImageNet}\\%
      \hline \hline
	AlexNetOWTBn& 57.1\\
	AlexNetOWTBn$^C$& 54.7\\
    BNet& 62.5\\
    BNet$^C$& 61.1\\
    ResNet50\footnote{Trained over $55$ epochs using a batch size of 128 on two TitanX with code publicly available and data augmentation specifically provided} & 67.3\\
	Dec$_8$ & 64.81\\
	\hline      
	Dec$_8$-640 & 66.87\\
	Dec$_8$-768 & 68.1\\
	\hline
	Ours-Bnet$^C$ & 62.7\\  	  	
  	Ours-Dec$_8$ & 64.8\\
  	Ours-Dec$_8$-640$_{sgs}$ & 67.5\\
  	Ours-Dec$_8$-640$_{gs}$ & 68.6\\
  	Ours-Dec$_8$-768 & 68.0\\
  	\hline  	  	 
   \end{tabular}
   \end{minipage}
  \end{table}



\begin{figure}
\begin{center}
\begin{minipage}[t]{.35\linewidth}
\vspace{0pt}
\centering
\includegraphics[width=\textwidth]{./figs/Bnet.png}
\end{minipage}%
\begin{minipage}[t]{.25\linewidth}
\vspace{0pt}
\centering
\begin{tabular}{ |l|c| }%
      \multicolumn{2}{c}{}\\
      \hline%
      \multicolumn{2}{|c|}{BNet$^C$ on ImageNet (in \%)} \\%
      \hline\hline
		&\multicolumn{1}{|c|}{GS} \\%
       \hline
    neuron& 12.70\\
    group-wise& 13.59\\
    within-group& 13.59\\
    total-induced & 25.58\\
    \hline
    relative acc. & 2.6\\
    \hline
    \end{tabular}%
\end{minipage}
\end{center}
\caption{Example results on ImageNet using BNet. The graph on the left shows the comparison on the number of neurons per layer between our approach and the baseline. Relative acc. refers to the relative improvement in performance with respect to the baseline.}
\label{fig:BNet} 
\end{figure}


 \begin{figure}
 \begin{center}
 \begin{minipage}[t]{.335\linewidth}
 \vspace{0pt}
 \centering
\hspace{-0.3cm}\includegraphics[width=\textwidth]{./figs/Dec8-640Places.png}
 \end{minipage}%
 \begin{minipage}[t]{.65\linewidth}
 \vspace{0pt}
 \centering
 \begin{tabular}{ cc }%
\hspace{-0.25cm}\begin{tabular}{ |l|c|c| }%
      \hline%
      \multicolumn{3}{|c|}{Dec$_8$-$640$ on Places2 (in \%)} \\%
      \hline \hline 
     &\multicolumn{1}{c|}{S-GS}&\multicolumn{1}{c|}{GS} \\%
     \hline
    neuron& 10.08&8.65\\
    group-wise& 11.40 & 9.80\\
    within-group& 17.99 & 9.80\\
    total-induced & 18.53&10.43\\
    \hline
    relative acc. & 1.31&1.88\\
    \hline      
    \end{tabular}%
&\hspace{-0.25cm}\begin{tabular}{ |l|c| }%
      \hline%
      \multicolumn{2}{|c|}{Top-1 acc (\%) on Places2}\\%
      \hline \hline
	AlexNetOWTBn& 44.5\\
	AlexNetOWTBn$^C$& 41.1\\
    BNet& 44.0\\
    BNet$^C$& 43.1\\
	Dec$_8$ & 46.6\\
	\hline      
	Ours-Dec$_8$-640$_{gs}$ & 47.6\\
  	Ours-Dec$_8$-640$_{sgs}$ & 47.3\\
\hline      
    \end{tabular}\\
(a)&(b)\\    
\end{tabular}%
 \end{minipage}
 \end{center}
 \caption{Experimental results on Places2. a) . b) Our results using DecomposeMe$_8$-$640$ on Places2 dataset. As shown there is a significant increment in the number of zeros on neurons with at least one non-zero valued parameter. c) Summary of state-of-the-art results on this dataset.}
 \label{fig:DecOnPlaces} 
 \end{figure}




% \begin{table}
% \caption{Experimental results on Places2. a) Our results using DecomposeMe$_8$-$640$ on Places2 dataset. As shown there is a significant increment in the number of zeros on neurons with at least one non-zero valued parameter. b) Summary of state-of-the-art results on this dataset.}
% \label{fig:DecOnPlaces} 
% \begin{tabular}{ cc }%
% \begin{tabular}{ |l|c|c| }%
%       \multicolumn{3}{c}{}\\
%       \hline%
%       \multicolumn{3}{|c|}{Dec$_8$-$640$ on Places2} \\%
%       \hline \hline 
%      &\multicolumn{1}{c|}{S-GS}&\multicolumn{1}{c|}{GS} \\%
%      \hline
%     neuron& 10.08\%&8.65\%\\
%     group-wise& 11.40\% & 9.80\%\\
%     within-group& 17.99\% & 9.80\%\\
%     total-induced & 18.53\%&10.43\%\\
%     \hline
%     relative acc. & 1.31\%&1.88\%\\
%     \hline      
%     \end{tabular}%
% &\begin{tabular}{ |l|c| }%
%       \hline%
%       \multicolumn{2}{|c|}{Top-1 acc (\%) on Places2}\\%
%       \hline \hline
% 	AlexNetOWTBn& 44.5\\
% 	AlexNetOWTBn$^C$& 41.1\\
%     BNet& 44.0\\
%     BNet$^C$& 43.1\\
% 	Dec$_8$ & 46.6\\
% 	\hline      
% 	Ours-Dec$_8$-640$_{gs}$ & 47.6\\
%   	Ours-Dec$_8$-640$_{sgs}$ & 47.3\\
% \hline      
%     \end{tabular}\\
% (a)&(b)\\    
% \end{tabular}%
% \end{table}




% \begin{table}[!t]
% \caption{Experimental results for ICDAR2003. zeros refers to the number of parameters set to zero in a non-zero kernel (as a l1-norm).}\label{tab:ICDAR}
% \centering
% {\small
% \begin{tabular}{c|c|cccccccc|c}
%       & Top-1 &Conv.& \multicolumn{4}{c}{Parameters} & \multicolumn{3}{c}{Reduction (\%)} & time\\
% Model & Acc.(\%) &kernels& Conv.& Linear &  Total & zeros & Kernel & Conv.  & All &  (ms) \\
% \hline
% baseline& 88.8 & 1584 &3694512  & 18432 & 3712944 & -- & -- & --& \\
% \hline
% Ours & 89.9 & 972 & 1019477 & 17352 &1036829 &1471914 & & & &\\
% \hline
% \end{tabular}
% }
% \end{table}


\begin{figure}
\begin{center}
\begin{minipage}[t]{.3\linewidth}
\vspace{0pt}
\centering
\hspace{-1.2cm}\includegraphics[width=1.2\textwidth]{./figs/ICDAR.png}
\end{minipage}%
\begin{minipage}[t]{.7\linewidth}
\vspace{0pt}
\centering
\begin{tabular}{ cc }
\begin{tabular}{ |l|c|c| }%
      \hline%
      \multicolumn{3}{|c|}{Dec$_{3}$ on ICDAR2003 (in \%)} \\%
      \hline\hline
		&\multicolumn{1}{c|}{S-GS}&\multicolumn{1}{c|}{GS} \\%
       \hline
    neuron& 38.64&55.11\\
    group-wise& 32.57&66.48\\
    within-group& 72.41&66.48 \\
    total-induced & 72.08&66.52\\
    \hline
    relative acc. & 1.24&1.38\\
    \hline      
    \end{tabular}      
    &\hspace{-0.25cm}\begin{tabular}{ |l|c| }%
      \hline%
      \multicolumn{2}{|c|}{Top-1 acc. on ICDAR2003}\\%
      \hline \hline
	MaxOut$_{Dec}$\footnote{Results from~\citet{Jaderberg148} using MaxOut layer instead of MaxPooling and decompositions as post-processing step}& 83.8\%\\
   	MaxOut\footnote{Results from~\citet{Jaderberg148}}& 89.8\%\\
   	MaxPool$_{2Dneurons}$& 83.8\%\\
	Dec$_3$ (baseline)& 89.3\%\\
	\hline      
	Ours-Dec$_{3-sgs}$ & 89.9\%\\
   	Ours-Dec$_{3-gs}$ & 90.1\%\\
\hline      
    \end{tabular}\\
(a)&(b)\\    
\end{tabular}        
\end{minipage}
\end{center}
\caption{Experimental results for ICDAR2003.}
\label{fig:ICDAR} 
\end{figure}

% \begin{table}[!t]
% \caption{Experimental results on ImageNet for DecomposeMe$_8^C$ and the baselines.}\label{tab:deepImageNet}
% \centering
% \begin{tabular}{L{0.5cm}lccc}
% &&\hspace{-0.015cm}Top-1 & \multicolumn{1}{c}{\#ConvP}  & \multicolumn{1}{c}{\#FCP}\\
% \hline
% &\hspace{-0.35cm}AlexNetOWTBn MatConvNet~\cite{VedaldiL14}&\hspace{-0.15cm}57.9 & 2.47M&58.6M\\
% &\hspace{-0.35cm}AlexNetOWTBn Baseline (retrain)&\hspace{-0.15cm}57.1 & 2.47M&58.6M\\[0.9ex]
% &\hspace{-0.35cm}AlexNetOWTBn$^C$&\hspace{-0.15cm}54.7& 2.47M&9.2M\\[0.9ex]
% \cline{2-5}
% &\hspace{-0.35cm}B-Net Baseline (VGG-B retrain)&\hspace{-0.15cm}62.5&9.4M&123.5M\\
% &\hspace{-0.35cm}B-Net$^C$&\hspace{-0.15cm}61.1&9.4M&25.0M\\[0.9ex]
% %\cline{3-8}\\
% \cline{2-5}
% &\hspace{-0.35cm}\textbf{DecomposeMe}$_8^{C}$&\hspace{-0.15cm}\textbf{65.4}&\textbf{7.0M}&\textbf{8.19M}\\[0.6ex]
% \hline
% \end{tabular}
% \end{table}
% \COMMENT{I Will add here a table with a comparison to the state of the art for the three datasets to state that we are producing 'state-of-the-art numbers. The table is filled with results obtained training from scratch existing networks. Basically the point is giving a direct comparison between Dec-8 with the rest (as it is giving quite good results 68.3\%, compared to 58 AlexNet) and summarizing the overall number of parameters at test time.}


\subsection{Benefits at test time}

\begin{table}
\begin{tabular}{ |l|c|c|c|c| }%
\hline
      \multicolumn{5}{|c|}{Relative Speed up (\%) on a single Tesla K20m}\\%
      \hline \hline      
      \multicolumn{1}{|c|}{}&\multicolumn{4}{c|}{Time }\\%
      \multicolumn{1}{|c|}{}&\multicolumn{4}{c|}{Batch Size}\\%
      \cline{2-5}
      \multicolumn{1}{|c|}{Model}&\multicolumn{1}{c|}{1}&\multicolumn{1}{c|}{2}&\multicolumn{1}{c|}{8}&\multicolumn{1}{c|}{16}\\%
      \hline
	Ours-BNet& 10.04&8.97&13.01&13.69\\
	Ours-Dec$_8$-640$_{gs}$ & -0.1 & 5.44 & 3.91&4.37\\
  	Ours-Dec$_8$-768$_{gs}$ & 15.29&17.11&15.99&15.62\\
    
    Ours-Dec$_{3gs}$&35.62&43.07&44.40&49.63\\
          \hline
    \end{tabular}
    \end{table}



\subsection{Discussion}
We need to comment on the need of keep training for a bit specially if the learning rate and the weight of the constraints are large. This is mainly to make sure the remaining parameters are properly adapted to the changes done. This is expected as we are modifying the parameters at the end of an epoch and it is aligned with the former algorithms optimal brain damage and optimal brain surgeon. Nevertheless, in most experiments, this is not a problem as a complete learning process involve a learning rate that continuously decreases towards zero. In our experiments on large scale dataset we do not experience that problem as after a few iterations the number of zeros is stabilized. 




As expected, marginal accuracy improvements happen when using AlexNet and VGG in their original form. This is mainly due to the presence of the fully connected layer which constantly compensates for differences happening in previous layers. However, our proposal significantly reduces the amount of memory and parameters needed and consequently, speeds-up at test time.

Significant improvements are obtained when fully connected layers are completely removed.

We have also empirically observed that the training-validation gap decreases when using fewer parameters.


\subsection{parameter sensitivity}
We focus now on the analysis of the sensitivity of the algorithm to the weights of the parameters. To this end, we represent in~\fig{} variations in performance and number of parameters (compared to a baseline) for different instances of our approach.

As shown, our algorithm systematically reduce the number of parameters while maintaining the performance. If additional savings are required, our approach significantly reduce the requirements while having minimal loss in performance (compared to optimal ones, that is, our best result).



==> oldText.tex <==
\section{Old Intro}
\COMMENT{Removed the filter decomposition approaches, since they do not really perform model selection, but rather build a more compact network. They will be discussed in related work, but I think this is not really the point here.}

\COMMENT{We focus on finding the optimal number of kernels per layer jointly within the training process}.
  
\COMMENT{Related work: No much, specially for Large-Scale, therefore it is important to focus on large Scale}.

\COMMENT{In the 90's for non-large scale (those approaches do not scale due to a Hessian computation): Optimal brain damage and optimal brain surgery}

\COMMENT{Related work should be categorized into: constructive (growing algorithms--i do not know any as width, only as depth), destructive or pruning algorithms: Distinguish here between pruning and distillation, and regularization based: common weight decay and the memory bounded}

\COMMENT{Additionally some comments on compression techniques, as ways to speed up the test phase of a conv. net -- maybe to state the relevance of the process}

\subsection{focus of current research}

Current methods focus on reducing fully connected layers which, when present, have the largest portion of parameters. However, a recent trend shows (and our experiments) that fully connected layers can be removed without penalizing the test accuracy (and with a significant reduction in the train-validation accuracy gap). This results definitely suggests that a large excess of parameters do incur in both overfitting and some accuracy penalties when they are not addressed properly.

While adding depth is effective it is also empirically proved that the additional layers produce marginal improvements (compared to the large amount of additional parameters) which suggest that most of these parameters are compensating overfitting while the rest basically aim at improving generalization performance.

Depth is well known to make a network more expressive. Over the last years, continuous efforts have been focused on improving learning algorithms for deep, very-deep and ultra-deep networks. The latest ones reaching hundreds of layers. While additional depth increases the performance if comes at a high price. Each layer significantly increases the number of parameters of the network and slows down the process. In addition, these additional layers difficult the training process due to exploding and vanishing gradients resulting in slow learning specially in the first layers. Finally, it has been empirically proved that these large deep models include a significant number of redundant parameters~\citet{DenilSDRF13}. In general the vast amount of computational resources and model complexity of these methods leads to marginal improvements in performance~\citet{ResNet2015}.


Current model selection is mostly achieved empirically. Some recent works have focused on optimizing the network architecture once it is trained. 
\subsection{our approach}
While recent efforts have successfully trained large networks, they do not explicitly exploit the hidden structure in the data (parameters).

In this paper, we explicitly address the structure of convolutional neural layers and aim at selecting the optimal model (while training) for a given task (e.g., classification in our experiments).

The algorithm considers each tensor as a group and aims at reducing groups with small entries (which effectively means reducing the size of the model). In our particular case of convolutional layers this has direct consequences in the computational requirements at test time in both memory and time.

Our algorithm addresses each layer independently and therefore is suited to handle different types of kernels as well as optimizes the output size which is specially relevant for domain transfer applications where the features of a network trained for a task (classification) are used for different tasks.

We aim at optimizing $f(\beta, X)= h(\beta, X) + g(\beta, X)$ where $\beta$ is the set of parameters. Common approaches limit the capacity of the network using parameter sparse inducing norms such as weight decay or $L_1$-norm. However, our interest is not in finding a few zeros at random positions within $\beta$ but we would like a solution that uses only a few groups (of parameters) in each layer. 


Our model selection proposal starts with a relatively wide network and then relies on regularization to obtain the optimal fit for the dataset at hand. 


\subsection{Major outcomes}
Given a limited network budget, our experiments suggests that there are better ways to use these parameters. Even with similar training size, these optimal models perform better than their counterparts. Furthermore, we expect larger improvements when the system keeps training for a longer period of time (as our models still exhibit lower training-validation accuracy gap).

At test time, constrained platforms do not perform well when the network is large as multiple operations need to be performed. Small platforms do not have large memory so efficiency there is a must.
We consistently improve overall accuracy (approx 3\% relative improvement) while reduce the number of parameters (up to 40\%) and, more importantly, fix the optimal structure of the network for a given task. At test time we obtain significant speeds-up and memory savings (not only due to the smaller network but due to the significant reduction in the number of feature maps computed).

\section{Old Related work}
\COMMENT{Is unit more general than (but equivalent to) channel?}
\COMMENT{JM: So, I guess unit is a bit of old terminology and now is equivalent to Neuron. A neuron is for instance a convolution kernel which is responsible for generating an output channel. A neuron comprises a set of parameters which 'act together' to produce an output.}


\COMMENT{In contrast with constructive methods, destructive approaches to model selection start with an initial deep network, and aim at reducing it while keeping its behavior unchanged. This trend was started by~\cite{damage} and \cite{BrainSurgeon}, who both relied on a notion of neuron saliency to remove the neurons that have little effect on the network output. This saliency measure, however, is derived from the network's Hessian, and thus does not easily scale to large architectures. The recent work of~\cite{distNets} can also be thought of as a destructive approach; it aims at learning a shallower network that mimics the behavior of an initial deep one, and thus ultimately reduces the number of parameters of the initial network. The main motivation of this work, however, was not truly model selection, but rather building a more compact network.}
\COMMENT{Are there more references for the destructive approach?}
\COMMENT{I only found references in the 90's or some really crap conference in the last 5 years:
http://arxiv.org/pdf/1512.03850.pdf https://hal.archives-ouvertes.fr/hal-01086842/document http://arxiv.org/pdf/1512.08571.pdf}


\COMMENT{This is the end of my version. It is quite a bit shorter, so check if I missed something. Also, feel free to add some more details.}



Model selection has not been widely addressed in this era of large scale systems. Currently, model selection is mostly done empirically with a lot of engineering efforts through exhaustive search over a set of possible network architectures. This approach has the obvious drawback of computational cost as many different networks need to be trained which is prohibitive especially for large scale problems. As a consequence, current approaches take advantage of some empirical results on a specific problem and reuse the architecture for the task at hand (for instance AlexNet and VGG have been adopted as main architectures over the last years). Nevertheless, historically, we can distinguish three different approaches to perform model selection in deep neural networks: constructive or incremental, destructive or pruning approaches and finally those based on regularization techniques. Incremental approaches were among the first attempts to reduce the complexity of exhaustive model search and consists of gradually growing the network. To this end, a small network is initially trained and then additional neurons are added while training. Initially, this approach was meant to grow the width of each layer. However, the current approach to a growing algorithm does not add neurons per layer while training but add layers once the small network has been trained. Examples of this approach are the common VGG (deep and very deep networks) where the smallest architecture is used to initialize the deeper ones. This has the additional advantage of dealing with the vanishing gradient problem as the initialization of the first layers is already a good one (from a pre-trained net). Moreover, additional layers do help in the regularization process. Nevertheless, it has been empirically shown that adding layers usually produce marginal improvements compared to the number of parameters being added.

A second group of works aiming at avoiding exhaustive model search is based on network pruning. The idea is starting with a large net and analyze the contribution of each neuron/parameter and trim where necessary \citet{damage,BrainSurgeon}. These approaches usually focus on analyzing the saliency of the weights and remove those which are irrelevant. For small datasets, two well-known algorithms in this area are: optimal brain damage~\citet{damage} and optimal brain surgeon~\citet{BrainSurgeon}. In optimal brain damage algorithm the number of parameters is reduced (for small scale classification problem) by about a factor of 4 while marginally improving generalization and significantly the training speed. However, this method is based on training a relative large network until some initial stopping criteria is reached and then compute second derivatives for each weight in the network removing the low-saliency ones. Then, train for a bit longer and repeat the basic steps until final convergence. This method requires the computation of the Hessian (the method assumes the Hessian matrix is diagonal) which is not practical in large scale problems. A different approach to determine the saliency of the weights is optimal brain surgeon~\citet{BrainSurgeon}. This method does not make specific assumptions on the Hessian but needs its computation. The main problem of optimal brain surgeon method is the evaluation of the contribution of individual weights is usually slow and therefore prohibitive for large scale problems. In any case, these two methods need to compute corrections once some parameters have been pruned to basically adjust the remaining weights. In the case of optimal brain surgeon, the inverse of the hessian also needs to be evaluated. 



Finally, the third group of works and most related to ours is based on regularization. These set of methods, in general, aim at penalizing complex architectures while training and perform network pruning through regularization. Common approaches in this area are weight decay, weight elimination and L$_1$ norm being weight decay the most widely used. Weight decay in a network can be formulated as:
\begin{equation}
E+\frac{\lambda}{2}\sum_i{w_i^2}
\end{equation}
\noindent where i loops over all the weights in the network. This regularization term favors small weights, and therefore, a network trained with this approach will tend to reduce the magnitude of the weights that are not contributing significantly to reduce the error of the model. One problem of this approach is that it tends to favor many small weights rather than a few larger ones (and therefore does not necessarily impose sparsity). Several modifications were introduced to overcome this problem such as weight elimination~\citet{WeightElimination}
\begin{equation}
E+\lambda\sum_i{\frac{w_i^2}{\hat{t^2}+w_i^2}}
\end{equation}
\noindent where $t$ is a fixed parameter which sets the a scale. This term will tend to favor a few larger weights and it is better than the simple weight-decay

Although these regularization techniques aim at pruning certain weights, they have been usually considered as an effective way to improve regularization~\citet{Krogh92asimple,Bartlett}



Our approach also starts with a relatively large network and gradually remove complete units while training proceeds. Similarly to brain surgeon and brain damage, our approach trains until certain criteria is reached (in our experiments, and without loss of generality, an epoch) and then regularizes the set of parameters being trained. 


Our approach does also start with a large network and gradually remove complete units while training. However, for practical reasons, in our case, the neurons are not physically removed from the architecture and therefore, the training time is not affected (improved). 





Within regularization methods, weight decay and l-1 norm have been used being weight decay the most widely used regularization together with early stopping. A combination of these two usually leads to limitations in the capacity of the network~\cite{}. In a similar way, data augmentation through adding noise has been widely exploited as regularization technique to improve generalization abilities of the network. However, none of them do take into account the distribution of the parameters in the network or within the layer (in filters), and none of them is specifically targeted to find the optimal model for the task at hand.

Recently, Collins and Kohli~\citet{CollinsKMemoryBounded14} used sparsity inducer techniques during training to reduce the memory footprint of a model. As a result they obtain a reduction up to a factor of four in the number of neurons with minimal loss in accuracy. Most of these parameters are concentrated within the fully connected layer and they perform layer-wise greedy search to reduce parameters within each convolutional layer. Furthermore, as they algorithm is focused on single parameters, the reduction is solely in the memory footprint of the parameters without speeds-up at test time. Contrary to those results, our experiments on large scale dataset demonstrate that it is possible to jointly reduce the number of neurons (not just parameters) significantly and still obtain a performance improvement. In addition, as we are considering neurons rather than isolated parameters, our reductions are directly translated into speed-ups at test time.



Additional works have proved the existence a large redundancy in the parameters of each kernel~\citet{DenilSDRF13}. In their work, Denil at al.~\citet{DenilSDRF13}  proved that only 5\% of the parameters of a filter are required to reconstruct the complete 2D kernel. However, most systems do have to reconstruct the square kernel to operate. In our work, we take advantage of the recent kernel decomposition architecture proposed in~\citet{} where the authors directly learn 1D kernels and therefore reduce significantly the number of parameters required. 

Finally, some additional work has been concentrated on speeding-up test time through model compression~\citet{Jaderberg14b,Fergus:NIPS2014}. Although it is not directly related to our work it is worth to mention that these methods do start with a pre-trained model and, in general, achieve decent speeds-up with, usually, some loss in accuracy. Moreover, these models act as a post-processing step. Contrary, we aim at directly training and selecting the model which is usually more attractive and more convenient~\citet{Srivastava:nips2015}. As demonstrated in our experiments, our approach is able to jointly learn the parameters and the model leading to optimal models in terms of memory savings, speeds-up at test time and improvements in the overall accuracy of the model.



Our main results are based on solely convolutional layers. Therefore, compared to AlexNet or VGG type of networks we directly remove the fully connected layers which are responsible for a vast portion of the parameters. While these last fully connected layers carry most of the parameters the former (convolutional layers) are slower computational wise and involve more memory during the computation (as feature maps are larger).




In the case of convolutional layers where parameters are organized in groups, the activation of the neuron depends in the complete group and not just a single parameter (as may happen in fully connected layers). Therefore, there is no straight relation between sparsity at parameter level and sparsity of the network. Nevertheless, setting a number of parameters to zero would reduce the effective capacity/flexibility of the system.




\subsection{Sparse group}
\COMMENT{I think I would write this using Eq.~\ref{sgs} as it is more generic; then specify $\alpha$ in the experiments. An additional benefit is that it would differ more for whatever I have seen or done in the past.}
\begin{equation}
min_W E + \lambda \sum_{l=1}^m{\sqrt{p_l}||W^l||_2},
\end{equation}
\noindent where $W^l$ is the set of parameters for the l-th layer.


\subsection{Sparse group sparse}
\citet{Simon13asparse-group}
\begin{equation}
\label{sgs}
min_W E + (1-\alpha)\lambda \sum_{l=1}^m{\sqrt{p_l}||W^l||_2 + \alpha\lambda||W||_1},
\end{equation}
\noindent where $\alpha \in [0,1]$. This is a combination between lasso and group-lasso penalties. When $\alpha=0$ we are optimizing group-sparsity as we did previously, while $\alpha=1$ turns out to be our a simple l-1 norm regularization.




==> supplementalmaterial.tex <==
\section{Additional Experiments}

\paragraph{Places2-401:} We now turn to the second large-scale image recognition dataset, Places 2. For this experiment, we focused on the Dec$_8$-640 architecture, trained with either the group sparsity regularizer or the sparse group Lasso one. Figure~\ref{fig:DecOnPlaces} summarizes our results and compares them with several baselines. These results are consistent with those obtained on ImageNet. The group sparsity regularizer reduces the total number of parameters by more than 10\%, and the sparse group Lasso yields an even greater reduction of $10\%$ of the neurons, which amounts to more than 18\% of the parameters. In both cases, the resulting network also leads to an improvement in top-1 accuracy. Importantly, this lets us outperform the current state-of-the-art on this dataset, even without using any advanced data augmentation technique such as color corrections or multiple crops at test time as in~\citep{ResNet2015,Krizhevsky_imagenetclassification}.
  
 \begin{figure}[t!]
 \begin{center}
 \begin{minipage}[t]{.335\linewidth}
 \vspace{0pt}
 \centering
\hspace{-0.3cm}\includegraphics[width=\textwidth]{./figs/Dec8-640Places_3.png}
 \end{minipage}%
 \begin{minipage}[t]{.65\linewidth}
 \vspace{0pt}
 \centering
 \begin{tabular}{ cc }%
\hspace{-0.25cm}\begin{tabular}{ |l|c|c| }%
      \hline%
      \multicolumn{3}{|c|}{Dec$_8$-$640$ on Places2 (in \%)} \\%
      \hline \hline 
     &\multicolumn{1}{c|}{SGL}&\multicolumn{1}{c|}{GS} \\%
     \hline
    neurons& 10.08&8.05\\
    group param& 11.40 & 9.18\\
    total param& 17.99 & 9.18\\
    total induced & 18.53&\ADDED{14.79}\\
    \hline
    accuracy gap & 1.31&1.88\\
    \hline      
    \end{tabular}%
&\hspace{-0.25cm}\begin{tabular}{ |l|c| }%
      \hline%
      \multicolumn{2}{|c|}{Top-1 acc (\%) on Places2}\\%
      \hline \hline
%	AlexNetOWTBn& 44.5\\
%	AlexNetOWTBn$^C$& 41.1\\
    BNet& 44.0\\
    BNet$^C$& 43.1\\
	Dec$_8$ & 46.6\\
    Dec$_8$-640 & 46.8\\
	\hline      
	Ours-Dec$_8$-640$_{GS}$ & 47.6\\
  	Ours-Dec$_8$-640$_{SGL}$ & 47.3\\
\hline      
    \end{tabular}\\
\end{tabular}%
 \end{minipage}
 \end{center}
 \vspace{-0.3cm}
 \caption{Experimental results on Places2-401 using Dec$_8$-$640$. From left to right, we show the reduction in number of neurons for each layer, the percentage of zeroed-out neuron/parameters, and the top-1 accuracy, compared to several baselines. Note that we achieve a significant reduction in number of parameters and, importantly, outperform the state-of-the-art on this dataset.}
 \label{fig:DecOnPlaces} 
 \end{figure}
